Multiscale Detection of Cancerous Tissue in High Resolution Slide Scans

We present an algorithm for multi-scale tumor (chimeric cell) detection in high resolution slide scans. The broad range of tumor sizes in our dataset pose a challenge for current Convolutional Neural Networks (CNN) which often fail when image features are very small (8 pixels). Our approach modifies the effective receptive field at different layers in a CNN so that objects with a broad range of varying scales can be detected in a single forward pass. We define rules for computing adaptive prior anchor boxes which we show are solvable under the equal proportion interval principle. Two mechanisms in our CNN architecture alleviate the effects of non-discriminative features prevalent in our data - a foveal detection algorithm that incorporates a cascade residual-inception module and a deconvolution module with additional context information. When integrated into a Single Shot MultiBox Detector (SSD), these additions permit more accurate detection of small-scale objects. The results permit efficient real-time analysis of medical images in pathology and related biomedical research fields.

==> fig-boxconfig.tex <==
  % \begin{figure}[h]
 % \centering
 % %\usepackage{graphicx}
%  \includegraphics[width=0.4\linewidth]{./images/jjj.eps}
%  \caption{The layout of homocentric Gt boxes and anchors. The dashed %boxes are the equal-proportion anchors with equal AR. The solid boxes %are object Gt boxes, where the red one is with the same AR to the %anchors.}\label{fig:boxconfig}
%\end{figure}



==> fig-origin.tex <==
\begin{figure}[h]
       \subfigure[tumor patch with context]{
       \label{fig:origin} %% label for first subfigure
       \includegraphics[width=0.4\linewidth]{./images/tumor-comparison1.eps}}
       %\hspace{1in}
       \subfigure[cropped tumor region]{
       \label{origin-inception} %% label for second subfigure
       \includegraphics[width=0.2\linewidth]{./images/tumor-comparison2.eps}}
      % \hspace{1in}
       \subfigure[human face]{
       \label{inception} %% label for second subfigure
       \includegraphics[width=0.2\linewidth]{./images/face-comparison1.eps}}
       \hspace{0.25in}
       \subfigure[cropped human face]{
       \label{inception-deconv} %% label for second subfigure
       \includegraphics[width=0.2\linewidth]{./images/face-comparison2.eps}}
       \caption{The comparison between detection of tumor and human face. We can see that both human faces can be easily detected no matter context. However, the tumor region without context is just a dark patch, extremely hard to detect.}
      \label{comparison-tumor-face} %% label for entire figure
      \end{figure}



==> fig-receptorfield.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.2\linewidth]{./images/ERF.eps}
\includegraphics[width=0.2\linewidth]{./images/tumor.eps}

\end{center}
   \caption{Gaussian distribution of effective receptive field:
   the black square and white region are
   theoretical receptive field and effective receptive field respectively.
   The brightness represents density.
   The figure is from \cite{luo2016understanding}. Our receptive field modification. (right)}
\label{fig:ERF}
\end{figure}




